Unsupervised Recalibration

Unsupervised recalibration (URC) is a general way to improve the accuracy of an already trained probabilistic classification or regression model upon encountering new data while deployed in the field. URC does not require any ground truth associated with the new field data. URC merely observes the model's predictions and recognizes when the training set is not representative of field data, and then corrects to remove any introduced bias. URC can be particularly useful when applied separately to different subpopulations observed in the field that were not considered as features when training the machine learning model. This makes it possible to exploit subpopulation information without retraining the model or even having ground truth for some or all subpopulations available. Additionally, if these subpopulations are the object of study, URC serves to determine the correct ground truth distributions for them, where naive aggregation methods, like averaging the model's predictions, systematically underestimate their differences.

==> sec-maths--depracated.tex <==
% Usage: \dev{X} (or simply \dev X) renders as X_dev.
\newcommand{\dev}[1]{{#1}_\text{dev}}
\newcommand{\app}[1]{{#1}_\text{app}}

\section{Global unsupervised recalibration}\label{sec:global_unsupervised_calibration}

	Consider a space of \textbf{features} $\mathcal X$ and space of \textbf{labels} $\mathcal Y=\{1, 2,\dots, n\}$. We are interested in a \textbf{classifier} $\func f {\mathcal X}{\mathbb R^n}$ predicting probabilities of labels $\mathcal Y$, i.e. if $x\in X$, then we want the $k$-th component of $f(x)$ vector to represent the chance that $f(x)$ represents class $k$.

	We can make this more precise by defining a probability space of all possible events $\Omega=\mathcal X\times \mathcal Y\times \mathcal T$. Here $\mathcal T = \{0, 1\}$ is a ``training indicator'' specifying which samples belong to the training data set. We make this statement precise later. 
	
	% We do not discuss any measurability issues, assuming that all sets and functions considered below are measurable.

On such space we define the following random variables:
\begin{itemize}
	\item $\func X \Omega {\mathcal X}$ is the projection giving features,
	\item $\func Y \Omega {\mathcal Y}$ is the projection giving labels,
	\item $\func T \Omega {\mathcal T}$ is the projection on the ``training indicator'' set. We identify this with the characteristic function of the training set, i.e. $(X\times Y)(T^{-1}(1))$ is the usual training data set $\{(x_i, y_i) \assuming i = 1, 2, \dots, m\}$,
	\item $\func C \Omega {\mathbb R^n}$ is the random variable representing $f$, i.e. $C = f\circ X$
		\begin{center}
			\begin{tikzcd}
				\Omega \arrow[rd, "C"] \arrow[d, "X", swap] \\
				\mathcal X \arrow[r, "f", swap]& \mathbb R^n
			\end{tikzcd}
		\end{center}
		By slight abuse of terminology we will refer to this random variable giving the classifier predictions as the \textbf{classifier} itself.
	\item $C_k\colon \Omega\to \mathbb R$ is the $k$-th component of $C$, i.e. $C_k=\pi_k\circ C$, where $\func{\pi_k}{\mathbb R^n}{\mathbb R}$ is the standard projection.
\end{itemize}

\begin{remark}
    We assume that the projections $X, Y, T$ and the classifier $C$ are measurable. This is enough to guarantee that all functions and sets considered below are measurable. 
\end{remark}



% Calibration on the training set
We say that a classifier is \textbf{calibrated on the training set} if $C_i$ describes the probability of $Y=i$ conditioned on $C$ and $T=1$, i.e. on the training set $T^{-1}(1)$ we have:
%
\begin{equation}\label{eq:cal_for_p}
    C_i\vert_{T^{-1}(1)} = P(Y=i \assuming T,\,C)\vert_{T^{-1}(1)}
\end{equation}
% Mention what me mean by conditional probability
As usual, the conditional probability of an event $Y=i$ conditioned on a random variable is the conditional expectation of the indicator function $1_{Y=i}$ conditioned on the random variable \citep{conditional-expectation}.

% Unbiased population
We call the training population \textbf{unbiased} for $Y$ if
%
\begin{equation}\label{eq:unbiased}
	P(Y=i \assuming T=1)=P(Y=i),
\end{equation}

% Calibrated overall
We would like to have a classifier that is \textbf{calibrated overall}, i.e.
\begin{equation}\label{eq:cal_overall}
	C_i = P(Y=i \assuming C).
\end{equation} 

\subsection{From training to practice}\label{ss:generalization_issues}
A classifier that is calibrated on the training set (eq. (\ref{eq:cal_for_p}) holds) may not be calibrated overall (eq. (\ref{eq:cal_overall}) does not hold) for two reasons.

%   Generalization issues, like overfitting. We suggest literature and don't pursue this direction
    First, classifier $C$ may pick up features specific to the training population only. There are various techniques reducing overfitting \citep{invariant-risk-minimization, overfitting} and we assume that the classifier $C$ was trained in a way that this is not a major problem.

%   Population is biased in some way.
    Second, the training population may be biased in some way, i.e. equation (\ref{eq:unbiased}) does not hold. This is common, since the training population often comes from a different source (where labels were available). Often, this is even deliberate in order to facilitate training, for example through stratification \citep{stratification}. 

\begin{example}[Entomologist's classifier]\label{ex:butterflies_setup}
    % Example -- butterflies and beatles
    Consider a classifier used to classify butterflies and beetles. As a simple feature space one can use wingspan and body weight. For simplicity assume that each of these features can take two values: ``small'' or ``large''.

    Equation (\ref{eq:cal_for_p}) states that a classifier was calibrated on the training data set. This means that if all we know is that a sample is from the training set and the classifier says ``beetle with 90\%'' (left hand side of eq. (\ref{eq:cal_for_p})), this chance is actually 90\% (right hand side). E.g. the classifier might only say this for ``small wings, large body", then 90\% of ``small wings, large body'' samples from the training set are actually beetles.

    If the training samples had been collected in a forest, beetles would be overrepresented compared to, say, a meadow. So the classifier is biased (eq. (\ref{eq:unbiased}) is does not hold): the chance to have a beetle in the training set (left hand side) is higher than overall (right hand side).

    Thus also equation (\ref{eq:cal_overall}) does not hold: $C_\text{beetle}$ is be too large and $C_\text{butterfly}$ is too low.
\end{example}

We consider such a bias as a miscalibration problem. This miscalibration is not of a form that most established parametric calibration techniques assume. This is because it stems not from the classifier being either simply overconfident \citep{platt-scaling} or underconfident \citep{beta-calibration}, but from the classifier systematically underestimating the probability of $Y=i$ in case $P(Y=i)>P(Y=i \assuming T=1)$ or systematically overestimating it in case $P(Y=i) < P(Y=i \assuming T=1)$.

Biased training sets are a known problem, and previous approaches aimed at quantifying and minimising that problem. For example, \citep{biasthroughstratification} suggest a sample stratification strategy that yields the minimax error considering an unknown bias. However, this error is still considerable, which is why we will aim at correcting it entirely.

\subsection{Independence assumption}\label{ss:independence}
To overcome this problem, we use an \textbf{independence assumption} that the bias is ``tame'':

\begin{itemize}
    \item Although the sample may be biased with respect to $Y$, the sample does not differ from the overall population with respect how $Y$ and $C$ interact: conditioned on each class $Y = i$, the distribution of $C$ is assumed to be identical in the training set and the real world, i.e.,
    \item $C$ and $T$ are \textit{relatively independent} given $Y$, i.e.,
    \item Axiom \ref{ax:independence} holds.
\end{itemize}

\begin{axiom}\label{ax:independence}
    Let $\mathcal A$ be the $\sigma$-algebra generated by $C$. We assume that for every $t\in \mathcal T$ and $\alpha\in \mathcal A$:
    \begin{equation}\label{eq:P_unbiased_for_C_rel_X}
        P(\alpha \wedge (T=t) \assuming Y=i) = P(\alpha \assuming Y=i) \cdot P(T=t \assuming Y=i)
    \end{equation}
\end{axiom}

 In many applications, this assumption is highly plausible since it already holds for the features $X$ used to compute $C$ -- for each class $Y=i$, the distribution of the features for members of this class does not differ between training set and overall population.

\begin{example}[Entomologist's classifier, continued]\label{ex:butterflies_independence}
    Distribution of features for a butterfly from the training set is probably the same (or quite close to) the distribution of features for a butterfly overall. If 40\% of butterflies from our trap have large wings and small bodies, then this is an acceptable estimate for the proportion of butterflies with large wings and small bodies overall. In contrast, just because 10\% of our sample set from the forest are butterflies, this doesn't mean that 10\% overall are butterflies.  
    
    Since the distribution of features are the same and the classifier is a function of the features, the distribution of classifier predictions for butterflies on the training set (left hand side of eq. (\ref{eq:cal_overall})) must also be the same as the distribution of classifier predictions for butterflies overall (right hand side).
\end{example}

\subsection{Global unsupervised recalibration for known bias}\label{ss:knownbias}
If the bias is known, recalibration is just accounting for this data shift.

\begin{lemma}\label{lemma:knownbias}
    Let unnormalized probabilities be random variables defined as
    \begin{equation}
        \bar{P}_i := C_i \cdot \frac{P(Y=i)}{P(Y=i\assuming T=1)}
    \end{equation}
    Then
    \begin{equation}
        P(Y=i\assuming C) = \frac{\bar{P}_i}{\sum\limits_j{\bar{P}_j}}
    \end{equation}
\end{lemma}

\begin{proof}
    Direct calculation.
\end{proof}

\subsection{Global unsupervised recalibration for unknown bias}\label{ss:global_recalibration_unknown_bias}
Due to lemma \ref{lemma:knownbias}, we need a sensible estimate for the true distribution of $Y$ in the population. A first pass might use the naive estimator:

\begin{definition}
    An unbiased estimator for the expected value $\mathbb{E}(C_i)$ is called a \textbf{naive estimator} for $P(Y = i)$.
\end{definition}

However, while useful for predicting the \textit{direction} of the bias given enough data, this will normally \textit{underestimate} the magnitude of the bias and will not approach the true value as the sample size increases:

\begin{theorem}\label{thm:naiveunderestimates}
    If
    \begin{equation}
        P(Y = i) < P(Y = i \assuming T),
    \end{equation}
    then
    \begin{equation}\label{eq:sandwich}
        P(Y = i) < \mathbb{E}(C_i) < P(Y = i \assuming T).
    \end{equation}
    The corresponding statement with $>$ also holds.
\end{theorem}

\begin{proof}
    \begin{align*}
        P(Y = i) & = \\
        & = \int P(Y = i \assuming C_i)\; \mathrm{d}C_i\\
        & < \int P(Y = i \assuming C_i \wedge T)\; \mathrm{d}C_i\\
        & = \mathbb{E}(C_i)
    \end{align*}
    The inequality holds pointwise for each $C_i$, as $C_i$ and $T$ are relatively independent given $Y$ and $P(Y = i) < P(Y = i|T)$ (equation \ref{eq:P_unbiased_for_C_rel_X}). This proves the first part of equation \ref{eq:sandwich}. For the second, we continue the chain of inequalities through
    \begin{align*}
        \mathbb{E}(C_i) & =\\
        & = \int P(Y = i \assuming C_i \wedge T)\; \mathrm{d}C_i \\
        & = \int P(Y = i \assuming C_i \wedge T)\; \mathrm{d}C_i \cdot \frac{\int P(T \wedge C_i)\; \mathrm{d}C_i}{P(T)}\\
        %& = \int P(Y = i | C_i & T) \mathrm{d}C_i \cdot \int P(T | C_i)\mathrm{d}C_i\\
        %& < \int P(Y = i | C_i & T) P(T | C_i)\mathrm{d}C_i\\
        %& < \int P(Y = i | C_i \wedge T) \mathrm{d}(C_i \wedge T)\\
        & < \int P(Y = i \assuming C_i \wedge T) \cdot \frac{P(T \wedge C_i)}{P(T)} \;\mathrm{d}C_i\\
        & = \int P(Y = i \assuming C_i \wedge T) \cdot \mathrm{d}(C_i \assuming T)\\
        & = P(Y = i \assuming T)
    \end{align*}
    Here, the inequality holds because $P(C_i \wedge T)$ is strictly increasing in $C_i$, as is $P(Y=i \assuming C_i\wedge T)$.
\end{proof}

If the classifier is very accurate, i.e. if $C_i(1-C_i) \approx 0$, then the naive estimator will be reasonably close to the desired $P(Y = i)$ (and the classifier will already be reasonably well calibrated to the field data). Otherwise, an alternative is needed.

Our alternative centers around partitioning classifier predictions into a finite number of clusters and analysing how often each cluster appears. We will then work backwards to determine which ground truth distribution might have caused these observations. The partition is a hyperparameter of URC.

\begin{definition}
    Call a family of sets $A=(A_i)_{i=1, 2, \dots, n}\subseteq\mathbb{R}^n$ a \textbf{partition for $C$} if:
    \begin{itemize}
        \item $P(C \in A_i \cap A_j) = 0$ for $i\neq j$ and
        \item $P\left(C \in \bigcup\limits_{i=1}^n A_i\right) = 1$. 
    \end{itemize}

    For a given partition $A$ of $C$, define  
    %
    \begin{equation}
        M_A = (P(C\in A_j \assuming Y=i \wedge T=1))_{i, j = 1, 2, \dots, n},
    \end{equation}
    %
    where each element $m_{i,j}$ of $M_A$ is the probability the classifier predicts an element of partition $j$ given an example of category $i$ in the training set. $M_{A}$ therefore encodes the distribution of predictions conditional on the ground truth. 
    
    Define further
    \begin{equation}
        \vec v_A =  (P(C\in A_j))_{j = 1, 2, \dots, n},
    \end{equation}
    where each entry $v_{A_j}$ of $\vec v_A$ is the probability the classifier predicts an element of partition $j$ in the field.
\end{definition}

The matrix $M_A$ is computed during the development phase. The vector $\vec v_A$ is observed in the field. These two include all the information URC requires to estimate the ground truth distribution in the field data (although a few extra summaries on the training data might be useful for regularisation, see remark \ref{rem:global_urc}, part 1).

The URC equations work for any partition\footnote{In fact, they generalize to a partition into more than $n$ sets.} of $C$. For reasons of numerical stability, it is sensible to choose a system of sets with similar probability and low variation. In the binary classification case, we suggest taking intervals which appear as equally likely from the training set. For a partition into $m$ intervals, this would mean for all $i\leq m$:
\begin{equation}\label{eq:example_partition}
    A_i = \left\{(y_1, y_2) \assuming y_1 + y_2 = 1 \wedge \frac{i-1}{m} < P(C_1 \leq y_1 \assuming T=1) \leq \frac{i}{m}\right\}
\end{equation}

\begin{lemma}\label{lemma:solvematrixeq}
    Let $(A_i)_{i=1, 2,..., n}\subseteq\mathbb{R}^n$ be a partition for $C$ and let
        \begin{equation*}
            \vec p_y = (P(Y=1), \dots, P(Y=n)).      
        \end{equation*}
    Then
    \begin{equation}
        M_A \cdot \vec p_y = \vec v_A
    \end{equation}
\end{lemma}

\begin{proof}
    Because of relative independence (equation (\ref{eq:P_unbiased_for_C_rel_X})),
    \begin{equation*}
        P(C\in A_j \assuming Y=i \wedge T=1) = P(C\in A_j \assuming Y=i).      
    \end{equation*}
    So the equation follows from case distinction on $Y=1 \vee ... \vee Y = n$.
\end{proof}

Lemma \ref{lemma:solvematrixeq} is an $n\times n$ system of linear equations relating the ground truth (which is not directly observable) to the model predictions (which are directly observable). $M_A$ is usually full rank (depending on the choice of partition), and then we could solve for $\vec p_x$.

But this is of limited use in practice: If the classifier is not very accurate, the condition number $\kappa$ of the above equation will be very high. Since sample limitations will usually leave at least some uncertainty when estimating the probability of $P(C\in A_j)$, lemma \ref{lemma:solvematrixeq} will not often narrow down $P(Y=i)$ in a meaningful way. In the case we extend our approach to partitions with more than $n$ members, this uncertainty will even lead to the (now over-determined) system normally being unsolvable when using the approximate values for $\vec v_A$.

However, it does give rise to an optimization problem. Instead of solving for $P(Y=i)$ directly, we can judge how likely a series of observations was for a candidate $P(Y=i)$. Define a loss function as follows.

\begin{definition}\label{def:Lll}
    For an unbiased sample $S$ and a partition $A$ for $C$, define a negative log-likelihood loss as $L_\mathrm{nll}: \left[0, 1\right]^n \rightarrow \mathbb{R}\cup\{\infty\}$ by
    \begin{equation}
        L_\mathrm{nll}(\vec{p}) = -\log B(|S|, (|S\wedge C\in A_i|)_{i = 1 ... n}, M_A \cdot \vec{p}),
    \end{equation}
    where $B(m, \vec{k}, \vec{p})$ is the multinomial mass function, i.e.
    \begin{equation}
        B(m, \vec{k}, \vec{p}) = {n \choose k_1, ..., k_n}p_1^{k_1}\cdot...\cdot p_n^{k_n}
    \end{equation}
\end{definition}

\begin{proposition}
    If $M_A$ is full rank, $L_\mathrm{nll}$ has a single global minimum, which for $|S|\rightarrow\infty$ converges against $\vec p_y$.
\end{proposition}
\begin{proof}
    The minimum of the multinomial function  $B(m, \vec k, \vec p)$ is attained at $\vec{p} = \vec{k} / m$, so in the limit case, where 
    \begin{equation}
        |(|S\wedge C\in A_i|)|/|S| \rightarrow P(C\in A_i),
    \end{equation}
    we approach $\vec p_y$, the solution of the equation in Lemma \ref{lemma:solvematrixeq}.
\end{proof}

Solving for minimal $L_\mathrm{nll}$ directly is risky due to the ill conditioned nature of $M_A$. To overcome this, we combine it with a regularization loss.

\begin{theorem}\label{thm:combinedloss}
    Let $L_\mathrm{reg}\colon [0, 1]^n\rightarrow\mathbb{R^+}\cup\{\infty\}$ be any $C^2$ function that fulfills
    \begin{equation*}
        L_\mathrm{reg}((P(Y=i))_{i=1, 2, ..., n})<\infty        
    \end{equation*}
    and let $M_A$ be full rank. 

The the global minimum of $L_\mathrm{nll} + L_\mathrm{reg}$:
\begin{enumerate}
    \item ... exists and is unique with arbitrarily high probability for sufficiently large $S$.
    \item ... converges in probability to $\vec p_y$ as $|S|\rightarrow\infty$.
    \item ... is the maximum a posteriori estimate \citep{maximumaposteriori} for $\vec p_y$ for fixed $T=1$ and prior probabilities proportional to $\exp L_\mathrm{reg}$.
\end{enumerate}
\end{theorem}

\begin{proof}
\begin{enumerate}
    \item Let $p<1$, we need to find an $k$ such that for $|S|\ge k$, the probability for unique existence of the minimum is at least $p$. Since $L_\mathrm{reg}$ is continuous, there is a compact neighborhood $U_1$ of $(P(Y=i))_{i=1...n}$ where $L_\mathrm{reg}<\infty$. By the extreme value theorem, there is a $b\in\mathbb{R}$ such that $(\frac{d}{dp_i})^2 L_\mathrm{reg}>b$ for all $i$ and in $U_1$. 
    
    The second derivative of the multinomial density $B$ in any direction is bounded from below by $|S|$, a value which is attained for $\vec{k} = (|S|, 0, ..., 0)$ and $\vec{p}=(1, 0, ..., 0)$. So for $|S|>-b$, the sum of the two losses is convex in $U_1$.
    
    Let $U_2\subset U_1$ be a compact neighborhood of $\vec p_y$ fully contained in the interior of $U_1$ such that the diameter of $U_2$ is smaller than the smallest distance of a point of $U_2$ to the boundary of $U_1$. Let $k_0$ be such that for $|S|>k_0$, the probability of the vector of ratios $v_r = (|(|S\wedge C\in A_i|)|/|S|)_{i=1...n}$ being in $U_2$ is at least $p$. 
    
    Since $U_1$ is compact and $L_\mathrm{reg}<\infty$ on $U_1$, the regularization loss has a maximum value $m_{U_1}$. Let $k_1 > k_0$ be such that for $|S|>k_1$, the negative log-likelihood loss of a vector being more than the diameter of $U_1$ away from the minimum $v_r$ is more than $m_{U_1}$ higher than the negative log-likelihood loss at that minimum. 
    
    Conditioned on $v_r \in U_2$, the combined loss at $v_r$ is smaller than at any point outside of $U_1$. As the combined loss is convex on $U_1$, there exists a unique global minimum. Since the event we conditioned in has probability at least $p$, so does the existence of a unique minimum.
    
    \item In the above, for any neighborhood $U_3\ni \vec p_y$, let $k_2>k_1$ be such that the probability of $v_r\in U_3\cap U_2$ is at least $p$. Then the global minimum is in $U_3$.
    
    \item The sum of the logarithms of likelihood and prior is minimized when the product of likelihood and prior is minimized, i.e. the posterior.
\end{enumerate}
\end{proof}

We propose to approximate this minimum and take it as estimator for the desired probabilities $\vec p_y$.

\begin{remark}\label{rem:global_urc}
\begin{enumerate}
    \item In our primary use case, we investigated different candidates for $L_\mathrm{reg}$. We settled on a loss proportional to the Kullback-Leibler divergence of the candidate $\vec p$ from the distribution observed on $T$, reasoning that the default assumption for the overall population should be one similar to $T$.
    \item While $|A|=n$ is necessary for solving the equation in lemma \ref{lemma:solvematrixeq}, it is not for optimizing a function as  \ref{thm:combinedloss}. It is perfectly reasonable to use partitions $A$ with more than $n$ elements, and indeed, in our primary use case, we had good experiences with $n=2$, $|A|=4$.
\end{enumerate}
\end{remark}

\section{Local unsupervised recalibration}\label{sec:local_unsupervised_calibration} 
Assume that when applying your trained probabilistic classifier $C$ for a random variable $Y\in\{1, 2, \dots, n\}$ in the field, you encounter a discrete random variable $G$, which you have not encountered before (for example $\Omega=\mathcal X\times \mathcal Y\times \mathcal T\times \mathcal G$, where $\mathcal G = \{1, 2, \dots, g\}$ and $G$ is a new feature indicating ``group'' to which observation belongs to, but not considered as a part of $\mathcal X$).
In some cases it is reasonable to assume that the different levels may have a different $P(Y=i|G=j)$, but that the relationship between $Y$ and $C$ is always the same in field samples.

\begin{example}[Entomologist's classifier once again]
    Consider two ``groups'' of insects: one of them have been caught close to the forest and the other close to the meadow.
    
    Maybe in forests beetles dominate while in meadow butterflies do, but the classifier cannot know this and account for this if not both groups were represented and recorded in the training set.
\end{example}

In that case, we can apply the global unsupervised recalibration procedure for each ``group'' individually, i.e. we recalibrate $C$ on $T=1 \wedge G = j$ in order to have an unbiased classifier on $G^{-1}(j)$ (see algorithm \ref{algo:urc_class}).

\begin{algorithm}[ht]
\label{algo:urc_class}
\SetAlgoLined
 partition predictions into sets using equation \ref{eq:example_partition}\;
 \For{each category (if separate categories are encountered in the field)}{
    get posterior ground truth distribution by minimizing the loss given in definition \ref{def:Lll} plus an optional regularizatition loss\;
    \For{each sample in category}{
    obtain calibrated probability by applying lemma \ref{lemma:knownbias}\;
    }
 }
 \caption{Unsupervised recalibration for classification}
\end{algorithm}

For levels of $G$ with few encountered examples, we will stay mainly with our priors. For levels with many examples, we will converge against the true values according to theorem \ref{thm:combinedloss}. 

The recalibrated classifier is then well calibrated for each level of $G$ individually for which there is sufficient data.

\section{Extension to regression}\label{sec:regression}

As usual, a regression model that produces a probability distribution can be calibrated by splitting the support of the distribution in $n$ intervals. The regression model is equivalent to a probabilistic classifier that gives a probability for each interval and individual regression models that give distributions within each interval conditioned on the event that the true value is in that interval. The probabilistic classifier is then recalibrated as described above.

Since such a classifier predicts an ordered categorical set, it makes sense to include a continuity component into $L_\mathrm{reg}$, i.e. $L_\mathrm{reg}$ should generally increase if $|C_i -C_{i+1}| \gg 0$.

Also, it makes sense to choose a partition based on intervals of the predicted overall value (which is a linear combination of the $C_i$). Analogous to equation (\ref{eq:example_partition}), our suggestion would be to split into $n$ quantiles (as observed on the training data).
